Incorporating Context into Subword Vocabularies

Most current popular subword tokenizers are trained based on word frequency statistics over a corpus, without considering information about co-occurrence or context. Nevertheless, the resulting vocabularies are used in language models' highly contextualized settings. We present SaGe, a tokenizer that tailors subwords for their downstream use by baking in the contextualized signal at the vocabulary creation phase. We show that SaGe does a better job than current widespread tokenizers in keeping token contexts cohesive, while not incurring a large price in terms of encoding efficiency or domain robustness. SaGe improves performance on English GLUE classification tasks as well as on NER, and on Inference and NER in Turkish, demonstrating its robustness to language properties such as morphological exponence and agglutination.

==> fig_lengths_all.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}{0.3\textwidth}
        \includegraphics[width=\textwidth]{Images/lengths_only.png}
        \caption{Light orange --- tokens that appear in \sage{} only, \\
        Light blue --- tokens that appear in \bpe{} only.}
        \label{fig:lengths-only}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.3\textwidth}
        \includegraphics[width=\textwidth]{Images/lengths_original.png}
        \caption{Orange --- final \sage{} of size 16K, \\
        Green --- Vanilla \bpe{} original vocabulary of size 20K.}
        \label{fig:lengths-original}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.3\textwidth}
        \includegraphics[width=\textwidth]{Images/lengths_final.png}
        \caption{Orange --- final \sage{} of size 16K, \\ Blue --- final Vanilla \bpe{} of size 16K.}        \label{fig:lengths-final}
    \end{subfigure}
    \caption{Tokens length distribution statistics of \bpe{} vs. \sage. (English)}
    \label{fig:lengths-all}
\end{figure*}



==> tab_xnli.tex <==

\begin{table}
    \centering
    \begin{tabular}{lrr}
        \toprule
         & \sage{} & \bpe{} \\
        \midrule
        Turkish & 51.83 & 47.90 \\
        \bottomrule
    \end{tabular}
    \caption{Performance (Acc \%) on XNLI task of BERT Turkish model trained on different subword vocabularies of size 16,000.}
    \label{tab:results-XNLI}
\end{table}

